A Scalable Sequential Framework for Dynamic Inverse Problems via Model Parameter Estimation

Large-scale dynamic inverse problems are often ill-posed due to model complexity and the high dimensionality of the unknown parameters. Regularization is commonly employed to mitigate ill-posedness by incorporating prior information and structural constraints. However, classical regularization formulations are frequently infeasible in this setting due to prohibitive memory requirements, necessitating sequential methods that process data and state information online, eliminating the need to form the full space-time problem. In this work, we propose a memory-efficient framework for reconstructing dynamic sequences of undersampled images from computerized tomography data that requires minimal hyperparameter tuning. The approach is based on a prior-informed, dimension-reduced Kalman filter with smoothing. While well suited for dynamic image reconstruction, practical deployment is challenging when the state transition model and covariance parameters must be initialized without prior knowledge and estimated in a single pass. To address these limitations, we integrate regularized motion models with expectation-maximization strategies for the estimation of state transition dynamics and error covariances within the Kalman filtering framework. We demonstrate the effectiveness of the proposed method through numerical experiments on limited-angle and single-shot computerized tomography problems, highlighting improvements in reconstruction accuracy, memory efficiency, and computational cost.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk --shell-escape -pdf \"$_[0]\"" );
    }
}

==> latexmkrc2 <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk --shell-escape -pdf \"$_[0]\"" );
    }
}

==> shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.

% Packages and macros go here
\usepackage[utf8]{inputenc}
\usepackage{xr-hyper}
% \usepackage{xr}
\usepackage{url}
\usepackage{soul}
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphics}
\usepackage{epstopdf}
\ifpdf
  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
\else
  \DeclareGraphicsExtensions{.eps}
\fi

% date 
\usepackage{datetime}
\newdateformat{monthyeardate}{%
  \monthname[\THEMONTH] \THEDAY, \THEYEAR}

% ORCID 
\usepackage{academicons}
\usepackage{xcolor}
\renewcommand{\orcid}[1]{\href{https://orcid.org/#1}{\textcolor[HTML]{A6CE39}{orcid.org/#1}}}

% math packages
% \usepackage{amsmath}
\allowdisplaybreaks
\usepackage{amssymb}
\usepackage{hyperref,cleveref}
\usepackage{commath}
\usepackage{mathtools}
\usepackage{bbm}

% figures
\usepackage{color}
\usepackage{graphicx}
\usepackage[small]{caption}
\usepackage{subcaption}

% Pseudocode, tables, and tikz 
\usepackage{relsize}
\usepackage{adjustbox}
\usepackage{algorithm,algpseudocode}
% \usepackage{algorithm}
% \usepackage[noend]{algpseudocode}
\usepackage{booktabs}
\usepackage{tikz}
%\usepackage[colorlinks=true]{hyperref}
\graphicspath{{figures/}}
% For comment blocks 
\usepackage{verbatim}

% Itemize with squares 
\renewcommand{\labelitemi}{\tiny$\blacksquare$}

% Prevent itemized lists from running into the left margin inside theorems and proofs
\usepackage{enumitem}
\setlist[enumerate]{leftmargin=.5in}
\setlist[itemize]{leftmargin=.5in}

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments 
\newsiamthm{problem}{Problem}
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis} 
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamremark{example}{Example}
\newsiamthm{claim}{Claim}
\newsiamthm{conjecture}{Conjecture}

% %% Other defined macros
% \makeatletter
% \newcommand*{\addFileDependency}[1]{
%   \typeout{(#1)}
%   \@addtofilelist{#1}
%   \IfFileExists{#1}{}{\typeout{No file #1.}}
% }
% \makeatother

% \newcommand*{\myexternaldocument}[1]{
%     \externaldocument{#1}
%     \addFileDependency{#1.tex}
%     \addFileDependency{#1.aux}
% }

%% Use \myexternaldocument on Overleaf
% \myexternaldocument{supplemental}

\usepackage[round]{natbib}  % Use 'round' for (Author, Year) style, or 'numbers' if you want [1]
\usepackage{url}
\usepackage[utf8]{inputenc} % Input encoding
\usepackage[T1]{fontenc}    % Font encoding
\usepackage{amsmath}        % For math environments
\usepackage{amssymb} 
\usepackage{graphicx}
\usepackage[margin=1in]{geometry}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{amsmath}
\usepackage{enumitem}% For math symbols
\usepackage{amsfonts}       % For \mathbb
\usepackage{graphicx}       % To include graphics (optional for outline, but good for final)
\usepackage[margin=1in]{geometry} % Set margins
\usepackage[svgnames]{xcolor} % Use colors, svgnames provides more predefined names
\usepackage{titlesec}       % To customize section titles
\usepackage{hyperref} 
\usepackage{amsmath}
\usepackage{url}
\usepackage{bm}
\usepackage{algorithm}
\usepackage{algpseudocode}
\usepackage{cite}
\usepackage{graphicx}  % Required for \includegraphics
\usepackage{subcaption} % Required for the subfigure environment
\usepackage{float} 
% For line numbers 
\usepackage{lineno}
\linenumbers

\newcommand{\va}{\boldsymbol{a}} % Use boldsymbol for Latin letters
\newcommand{\vb}{\boldsymbol{b}} % Use boldsymbol for Latin letters
\newcommand{\vc}{\boldsymbol{c}} % Use boldsymbol for Latin letters
\newcommand{\vd}{\boldsymbol{d}} % Use boldsymbol for Latin letters
\newcommand{\ve}{\boldsymbol{e}} % Use boldsymbol for Latin letters
\newcommand{\vf}{\boldsymbol{f}} % Use boldsymbol for Latin letters
\newcommand{\vg}{\boldsymbol{g}} % Use boldsymbol for Latin letters
\newcommand{\vh}{\boldsymbol{h}} % Use boldsymbol for Latin letters
\newcommand{\vi}{\boldsymbol{i}} % Use boldsymbol for Latin letters
\newcommand{\vj}{\boldsymbol{j}} % Use boldsymbol for Latin letters
\newcommand{\vk}{\boldsymbol{k}} % Use boldsymbol for Latin letters
\newcommand{\vl}{\boldsymbol{l}} % Use boldsymbol for Latin letters
\newcommand{\vm}{\boldsymbol{m}} % Use boldsymbol for Latin letters
\newcommand{\vn}{\boldsymbol{n}} % Use boldsymbol for Latin letters
\newcommand{\vo}{\boldsymbol{o}} % Use boldsymbol for Latin letters
\newcommand{\vp}{\boldsymbol{p}} % Use boldsymbol for Latin letters
\newcommand{\vq}{\boldsymbol{q}} % Use boldsymbol for Latin letters
\newcommand{\vr}{\boldsymbol{r}} % Use boldsymbol for Latin letters
\newcommand{\vs}{\boldsymbol{s}} % Use boldsymbol for Latin letters
\newcommand{\vt}{\boldsymbol{t}} % Use boldsymbol for Latin letters
\newcommand{\vu}{\boldsymbol{u}} % Use boldsymbol for Latin letters
\newcommand{\vv}{\boldsymbol{v}} % Use boldsymbol for Latin letters



\newcommand{\vF}{\boldsymbol{F}} % Use boldsymbol for Latin letters

\newcommand{\vJ}{\boldsymbol{J}} % Use boldsymbol for Latin letters

\newcommand{\vO}{\boldsymbol{O}} % Use boldsymbol for Latin letters

\newcommand{\vV}{\boldsymbol{V}} % Use boldsymbol for Latin letters

\newcommand{\vX}{\boldsymbol{X}} % Use boldsymbol for Latin letters
\newcommand{\vY}{\boldsymbol{Y}} % Use boldsymbol for Latin letters


% Greek Lowercase Letters
\newcommand{\valpha}{\boldsymbol{\alpha}} % Use boldsymbol for Greek letters
\newcommand{\vbeta}{\boldsymbol{\beta}} % Use boldsymbol for Greek letters
\newcommand{\vgamma}{\boldsymbol{\gamma}} % Use boldsymbol for Greek letters
\newcommand{\vdelta}{\boldsymbol{\delta}} % Use boldsymbol for Greek letters
\newcommand{\vepsilon}{\boldsymbol{\epsilon}} % Use boldsymbol for Greek letters
\newcommand{\vzeta}{\boldsymbol{\zeta}} % Use boldsymbol for Greek letters
\newcommand{\veta}{\boldsymbol{\eta}} % Use boldsymbol for Greek letters
\newcommand{\vtheta}{\boldsymbol{\theta}} % Use boldsymbol for Greek letters
\newcommand{\viota}{\boldsymbol{\iota}} % Use boldsymbol for Greek letters
\newcommand{\vkappa}{\boldsymbol{\kappa}} % Use boldsymbol for Greek letters
\newcommand{\vlambda}{\boldsymbol{\lambda}} % Use boldsymbol for Greek letters
\newcommand{\vmu}{\boldsymbol{\mu}} % Use boldsymbol for Greek letters
\newcommand{\vnu}{\boldsymbol{\nu}} % Use boldsymbol for Greek letters

\newcommand{\vpi}{\boldsymbol{\pi}} % Use boldsymbol for Greek letters
\newcommand{\vrho}{\boldsymbol{\rho}} % Use boldsymbol for Greek letters
\newcommand{\vsigma}{\boldsymbol{\sigma}} % Use boldsymbol for Greek letters
\newcommand{\vtau}{\boldsymbol{\tau}} % Use boldsymbol for Greek letters
\newcommand{\vupsilon}{\boldsymbol{\upsilon}} % Use boldsymbol for Greek letters
\newcommand{\vphi}{\boldsymbol{\phi}} % Use boldsymbol for Greek letters
\newcommand{\vchi}{\boldsymbol{\chi}} % Use boldsymbol for Greek letters
\newcommand{\vpsi}{\boldsymbol{\psi}} % Use boldsymbol for Greek letters
\newcommand{\vomega}{\boldsymbol{\omega}} % Use boldsymbol for Greek letters

% Greek Uppercase Letters
\newcommand{\vAlpha}{\boldsymbol{A}} % Use boldsymbol for Greek letters (often Latin equivalent)
\newcommand{\vBeta}{\boldsymbol{B}} % Use boldsymbol for Greek letters (often Latin equivalent)
\newcommand{\vGamma}{\boldsymbol{\Gamma}} % Use boldsymbol for Greek letters
\newcommand{\vDelta}{\boldsymbol{\Delta}} % Use boldsymbol for Greek letters
\newcommand{\vEpsilon}{\boldsymbol{E}} % Use boldsymbol for Greek letters (often Latin equivalent)
\newcommand{\vZeta}{\boldsymbol{Z}} % Use boldsymbol for Greek letters (often Latin equivalent)
\newcommand{\vEta}{\boldsymbol{H}} % Use boldsymbol for Greek letters (often Latin equivalent)
\newcommand{\vTheta}{\boldsymbol{\Theta}} % Use boldsymbol for Greek letters
\newcommand{\vIota}{\boldsymbol{I}} % Use boldsymbol for Greek letters (often Latin equivalent)
\newcommand{\vKappa}{\boldsymbol{K}} % Use boldsymbol for Greek letters (often Latin equivalent)
\newcommand{\vLambda}{\boldsymbol{\Lambda}} % Use boldsymbol for Greek letters
\newcommand{\vMu}{\boldsymbol{M}} % Use boldsymbol for Greek letters (often Latin equivalent)
\newcommand{\vNu}{\boldsymbol{N}} % Use boldsymbol for Greek letters (often Latin equivalent)
\newcommand{\vXi}{\boldsymbol{\Xi}} % Use boldsymbol for Greek letters
\newcommand{\vOmicron}{\boldsymbol{O}} % Use boldsymbol for Greek letters (often Latin equivalent)
\newcommand{\vPi}{\boldsymbol{\Pi}} % Use boldsymbol for Greek letters
\newcommand{\vRho}{\boldsymbol{P}} % Use boldsymbol for Greek letters (often Latin equivalent)
\newcommand{\vSigma}{\boldsymbol{\Sigma}} % Use boldsymbol for Greek letters
\newcommand{\vTau}{\boldsymbol{T}} % Use boldsymbol for Greek letters (often Latin equivalent)
\newcommand{\vUpsilon}{\boldsymbol{\Upsilon}} % Use boldsymbol for Greek letters
\newcommand{\vPhi}{\boldsymbol{\Phi}} % Use boldsymbol for Greek letters
\newcommand{\vChi}{\boldsymbol{X}} % Use boldsymbol for Greek letters (often Latin equivalent)
\newcommand{\vPsi}{\boldsymbol{\Psi}} % Use boldsymbol for Greek letters
\newcommand{\vOmega}{\boldsymbol{\Omega}} % Use boldsymbol for Greek letters


% %% Added on Overleaf: enabling xr
% \makeatletter
% \newcommand*{\addFileDependency}[1]{% argument=file name and extension
%   \typeout{(#1)}% latexmk will find this if $recorder=0 (however, in that case, it will ignore #1 if it is a .aux or .pdf file etc and it exists! if it doesn't exist, it will appear in the list of dependents regardless)
%   \@addtofilelist{#1}% if you want it to appear in \listfiles, not really necessary and latexmk doesn't use this
%   \IfFileExists{#1}{}{\typeout{No file #1.}}% latexmk will find this message if #1 doesn't exist (yet)
% }
% \makeatother

% \newcommand*{\myexternaldocument}[1]{%
%     \externaldocument{#1}%
%     \addFileDependency{#1.tex}%
%     \addFileDependency{#1.aux}%
% }




% % SIAM Shared Information Template
% % This is information that is shared between the main document and any
% % supplement. If no supplement is required, then this information can
% % be included directly in the main document.

% % Packages and macros go here
% \usepackage[utf8]{inputenc}
% \usepackage{xr-hyper}
% % \usepackage{xr}
% \usepackage{url}
% \usepackage{soul}
% \usepackage{lipsum}
% \usepackage{amsfonts}
% \usepackage{graphics}
% \usepackage{epstopdf}
% \ifpdf
%   \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
% \else
%   \DeclareGraphicsExtensions{.eps}
% \fi

% % date 
% \usepackage{datetime}
% \newdateformat{monthyeardate}{%
%   \monthname[\THEMONTH] \THEDAY, \THEYEAR}

% % ORCID 
% \usepackage{academicons}
% \usepackage{xcolor}
% \renewcommand{\orcid}[1]{\href{https://orcid.org/#1}{\textcolor[HTML]{A6CE39}{orcid.org/#1}}}
% \newcommand{\MP}[1]{{\color{cyan}#1}}
% % math packages
% \usepackage{amsmath}
% \allowdisplaybreaks
% \usepackage{amssymb}
% \usepackage{hyperref,cleveref}
% \usepackage{commath}
% \usepackage{mathtools}
% \usepackage{bbm}
% \newcommand{\vx}{\mathbf{x}}
% \newcommand{\vy}{\mathbf{y}}
% \newcommand{\vH}{\mathbf{H}}
% \newcommand{\vR}{\mathbf{R}}
% \newcommand{\vQ}{\mathbf{Q}}
% \newcommand{\vM}{\mathbf{M}}
% \newcommand{\vC}{\mathbf{C}}
% \newcommand{\vP}{\mathbf{P}}
% \newcommand{\vS}{\mathbf{S}}
% \newcommand{\vU}{\mathbf{U}}
% \newcommand{\vI}{\mathbf{I}}
% \newcommand{\vB}{\mathbf{B}}
% \newcommand{\vA}{\mathbf{A}}
% \newcommand{\vD}{\mathbf{D}}
% \newcommand{\vK}{\mathbf{K}}
% \newcommand{\vL}{\mathbf{L}}
% \newcommand{\vG}{\mathbf{G}}
% \newcommand{\vT}{\mathbf{T}}
% \newcommand{\vN}{\mathbf{N}}
% \newcommand{\vE}{\mathbf{E}}
% \newcommand{\vZ}{\mathbf{Z}}
% \newcommand{\vW}{\mathbf{W}}
% \newcommand{\vxi}{\boldsymbol{\xi}} % Use 
% % figures
% \usepackage{color}
% \usepackage{graphicx}
% \usepackage[small]{caption}
% \usepackage{subcaption}

% % Pseudocode, tables, and tikz 
% \usepackage{relsize}
% \usepackage{adjustbox}
% \usepackage{algorithm,algpseudocode}
% % \usepackage{algorithm}
% % \usepackage[noend]{algpseudocode}
% \usepackage{booktabs}
% \usepackage{tikz}
% %\usepackage[colorlinks=true]{hyperref}
% \graphicspath{{figures/}}
% % For comment blocks 
% \usepackage{verbatim}

% % Itemize with squares 
% \renewcommand{\labelitemi}{\tiny$\blacksquare$}

% % Prevent itemized lists from running into the left margin inside theorems and proofs
% \usepackage{enumitem}
% \setlist[enumerate]{leftmargin=.5in}
% \setlist[itemize]{leftmargin=.5in}

% % Add a serial/Oxford comma by default.
% \newcommand{\creflastconjunction}{, and~}

% % Used for creating new theorem and remark environments 
% \newsiamthm{problem}{Problem}
% \newsiamremark{remark}{Remark}
% \newsiamremark{hypothesis}{Hypothesis} 
% \crefname{hypothesis}{Hypothesis}{Hypotheses}
% \newsiamremark{example}{Example}
% \newsiamthm{claim}{Claim}
% \newsiamthm{conjecture}{Conjecture}

% % %% Other defined macros
% % \makeatletter
% % \newcommand*{\addFileDependency}[1]{
% %   \typeout{(#1)}
% %   \@addtofilelist{#1}
% %   \IfFileExists{#1}{}{\typeout{No file #1.}}
% % }
% % \makeatother

% % \newcommand*{\myexternaldocument}[1]{
% %     \externaldocument{#1}
% %     \addFileDependency{#1.tex}
% %     \addFileDependency{#1.aux}
% % }


% % %% Added on Overleaf: enabling xr
% % \makeatletter
% % \newcommand*{\addFileDependency}[1]{% argument=file name and extension
% %   \typeout{(#1)}% latexmk will find this if $recorder=0 (however, in that case, it will ignore #1 if it is a .aux or .pdf file etc and it exists! if it doesn't exist, it will appear in the list of dependents regardless)
% %   \@addtofilelist{#1}% if you want it to appear in \listfiles, not really necessary and latexmk doesn't use this
% %   \IfFileExists{#1}{}{\typeout{No file #1.}}% latexmk will find this message if #1 doesn't exist (yet)
% % }
% % \makeatother

% % \newcommand*{\myexternaldocument}[1]{%
% %     \externaldocument{#1}%
% %     \addFileDependency{#1.tex}%
% %     \addFileDependency{#1.aux}%
% % }

% % Sets running headers as well as PDF title and authors

\headers{Reduced Kalman Filter via Model Parameter Estimation}{A.\ Keating, M.\ Pasha}

\title{Iterative Optical Flow For Reduced Kalman Filtering and Smoothing
\thanks{
\monthyeardate\today 
\corresponding{Mirjeta Pasha} 
}}

\author{
Aryeh Keating\thanks{Department of Mathematics \& Academy of Data Science, Virginia Tech, USA, (\email{aryehkeating@vt.edu}; \email{mpasha@vt.edu}, \orcid{0000-0003-4249-2421})} 
\and 
Mirjeta Pasha\footnotemark[2] 
}


\renewcommand{\t} {^{\top}}                                % transpose, e.g. $A\t$
\renewcommand{\d} {{\rm d}}                                % differential d
\renewcommand{\H} {^{{\rm H}}}                             % Hermitian
\renewcommand{\vec}[1] {{\rm vec}(#1)}                     % vectorize matrix
\newcommand{\inner} [2]{\langle #1,#2\rangle}           % f.e. \inner product[\infty]{A-B}
% \newcommand{\norm} [2][]{\left\|#2\right\|_{#1}}           % f.e. \norm[\infty]{A-B}
% \newcommand{\abs}  [2][]{\left|#2\right|_{#1}}             % f.e. \abs[\infty]{A-B}
\newcommand{\cond} [2][]{{\rm cond}_{#1}\left( #2 \right)} % f.e. \cond[\infty]{A}
\newcommand{\pow}  [1]  {^{\left(#1\right)}}               % brackets exponent
\newcommand{\sign} [1]  {{\rm sign\!}\left( #1 \right)}    % signum
\newcommand{\rank} [1]  {{\rm rank\!}\left( #1 \right)}    % rank of a matrix
\newcommand{\diag} [1]  {{\rm diag\!}\left( #1 \right)}    % diagonal of a matrix
\newcommand{\spann}[1]  {{\rm span\!}\left( #1 \right)}    % span of a function % Careful \span conflicts 
\usepackage{amsopn}









% Declare the float 'algorithm' + new environment 'algo' 
%=====================================================================
\usepackage{ifthen}
\usepackage{float}
\floatstyle{ruled}
\newfloat{algorithm}{htb}{alg}%[section]
\floatname{algorithm}{Algorithm}
%\newcommand{\listofalgorithms}{\listof{algorithm}{Algorithms}}
%=====================================================================
% Define the new environment 'algorithmic' and some related stuff
%---------------------------------------------------------------------
%
% row index
\newcounter{algo@row}
%
% row indent (x 1cc)
\newcounter{algo@rowindent}
%
% default numbering & font
\newcommand{\algofont}[1]{\textbf{#1}}% S1
\newcommand{\algonumbersize}[1]{\scriptsize{#1}}% S2
\newcommand{\algopreitem}[1][\arabic{algo@row}]{\texttt{\algonumbersize{#1}}}
\newcommand{\algoitemskip}{\hspace{\value{algo@rowindent}cc}}
%
% shift row numbering
\newcommand{\algoskipline}[1]{\addtocounter{algo@row}{#1}}% S3
\newcommand{\algosetline}[1]{\setcounter{algo@row}{#1}\addtocounter{algo@row}{-1}}% S3
\newcommand{\algoskipindent}[1]{\addtocounter{algo@rowindent}{#1}}% S3
%
%---------------------------------------------------------------------
%
% environment
\newenvironment{algo}{\vskip.3em\small%
	\begin{list}{\algopreitem\texttt{\algonumbersize{:}}}{%
			\usecounter{algo@row}%
			\setcounter{algo@rowindent}{0}%
			\setlength{\itemindent}{2em}%
			\setlength{\labelwidth}{2em}% indent=1em
			\setlength{\parsep}{0cm}%
		}%
	}{
	\end{list}%\vskip-.5em
}
%
%---------------------------------------------------------------------
%
% open alg-nested-environment
\newcommand{\algonewnestedopen}[2]{
	\newcommand{#1}[1][]{%
		\ifthenelse{\equal{##1}{}}{\item}{\item[{\algopreitem[##1]}]}
		\algoitemskip\algofont{#2}%
		\addtocounter{algo@rowindent}{1}%
		\ignorespaces
	}
}
%
% alg-nested-environment aux
\newcommand{\algonewnestedaux}[2]{
	\newcommand{#1}[1][]{
		\addtocounter{algo@rowindent}{-1}
		\ifthenelse{\equal{##1}{}}{\item}{\item[{\algopreitem[##1]}]}
		\algoitemskip\algofont{#2}%
		\addtocounter{algo@rowindent}{+1}%
		\ignorespaces
	}
}
%
% close alg-nested-environment
\newcommand{\algonewnestedclose}[2]{
	\newcommand{#1}[1][]{
		\addtocounter{algo@rowindent}{-1}
		\ifthenelse{\equal{##1}{}}{\item}{\item[{\algopreitem[##1]}]}
		\algoitemskip\algofont{#2}%
		\ignorespaces
	}
}
%
% define new command
\newcommand{\algonewcommand}[2]{
	\newcommand{#1}[1][default]{
		\ifthenelse{\equal{##1}{default}}{\item}{\item[{\algopreitem[##1]}]}%
		\algoitemskip\algofont{#2}%
		\ignorespaces
	}%
}
%
% define new keyword
\newcommand{\algonewkeyword}[2]{\newcommand{#1}{\algofont{#2}}}
%
%=====================================================================
% Standard definitions for 'algorithmic'
%---------------------------------------------------------------------
%
% standard statement
\algonewcommand{\STATE}{\ignorespaces}
%
% 'Input and Output' statement
\algonewcommand{\INPUT}{Input: }
% \algonewcommand{\OUTPUT}{Output: }
\algonewcommand{\pINPUT}{\phantom{Input: }}
%
% 'Compute' statement
\algonewcommand{\COMPUTE}{Compute: }
%
% 'Output' statement
\algonewcommand{\OUTPUT}{Output: }
\algonewcommand{\pOUTPUT}{\phantom{Output: }}



%
% 'if' loop
\algonewnestedopen{\IF}{if }
\algonewnestedaux{\ELSEIF}{else if }
\algonewnestedaux{\ELSE}{else }
\algonewnestedclose{\ENDIF}{end if }
%
% 'for' loop
\algonewnestedopen{\FOR}{for }
\algonewnestedclose{\ENDFOR}{end for }
%

% 'while' loop
\algonewnestedopen{\WHILE}{while }
\algonewnestedclose{\ENDWHILE}{end while }
%
% 'break'
\algonewcommand{\BREAK}{break}%

%
% keywords (no indent, no new line)
% \algonewkeyword{\For}{for }%
\algonewkeyword{\To}{to }%
\algonewkeyword{\Do}{do }%
% \algonewkeyword{\If}{if }%
\algonewkeyword{\Then}{then }%
% \algonewkeyword{\Else}{else }%
\algonewkeyword{\End}{end }%
\algonewkeyword{\AND}{and }%
\algonewkeyword{\True}{true }%
\algonewkeyword{\False}{false }%
% \algonewkeyword{\Call}{call }%
\algonewkeyword{\irbleigs}{irbleigs }%
\algonewkeyword{\tridiag}{tridiag}%
\algonewkeyword{\reorth}{reorth}%
%=====================================================================

% commands 
\newcommand{\todo}[1]{{\Large \textcolor{red}{#1}}}
\newcommand{\revA}[1]{{\color{red}#1}}
\newcommand{\revB}[1]{{\color{blue}#1}}
\newcommand{\revC}[1]{{\color{cyan}#1}}
\newcommand{\JG}[1]{{\color{red}#1}}
\newcommand{\MP}[1]{{\color{cyan}#1}}
\newcommand{\JL}[1]{{\color{blue}#1}}
% definitions 
\newcommand{\MAP}{\mathrm{MAP}}
\DeclareMathOperator*{\argmin}{arg\,min} 
\DeclareMathOperator*{\argmax}{arg\,max} 
% \DeclareMathOperator{\rank}{rank}
% \DeclareMathOperator{\diag}{diag}
\newcommand{\scp}[2]{\left\langle{#1, #2}\right\rangle} 
\newcommand{\Span}{\mathrm{span}}
\newcommand{\LS}{\mathrm{LS}}
\renewcommand{\dim}{\mathrm{dim} \,}
\renewcommand{\d}{\mathrm{d}}
\newcommand{\intd}{\, \mathrm{d}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\R}{\mathbb{R}} 

\newcommand{\fnum}{f^{\operatorname{num}}} 
\newcommand{\fvol}{f^{\operatorname{Vol}}} 
\newcommand{\fnumo}{f^{\operatorname{num}}_1} 
\newcommand{\fnumt}{f^{\operatorname{num}}_2} 
\newcommand{\bA}{{\bf A}}
\newcommand{\bB}{{\bf B}}
\newcommand{\bC}{{\bf C}}
\newcommand{\bD}{{\bf D}}
\newcommand{\bE}{{\bf E}}
\newcommand{\bF}{{\bf F}}
\newcommand{\bG}{{\bf G}}
\newcommand{\bH}{{\bf H}}
\newcommand{\bI}{{\bf I}}
\newcommand{\bJ}{{\bf J}}
\newcommand{\bK}{{\bf K}}
\newcommand{\bL}{{\bf L}}
\newcommand{\bM}{{\bf M}}
\newcommand{\bN}{{\bf N}}
\newcommand{\bO}{{\bf O}}
\newcommand{\bP}{{\bf P}}
\newcommand{\bQ}{{\bf Q}}
\newcommand{\bR}{{\bf R}}
\newcommand{\bS}{{\bf S}}
\newcommand{\bT}{{\bf T}}
\newcommand{\bU}{{\bf U}}
\newcommand{\bV}{{\bf V}}
\newcommand{\bW}{{\bf W}}
\newcommand{\bX}{{\bf X}}
\newcommand{\bY}{{\bf Y}}
\newcommand{\bZ}{{\bf Z}}
\newcommand{\ba}{{\bf a}}
\newcommand{\bb}{{\bf b}}
\newcommand{\bc}{{\bf c}}
\newcommand{\bd}{{\bf d}}
\newcommand{\be}{{\bf e}}
\newcommand{\bff}{{\bf f}}
\newcommand{\bg}{{\bf g}}
\newcommand{\bh}{{\bf h}}
\newcommand{\bi}{{\bf i}}
\newcommand{\bj}{{\bf j}}
\newcommand{\bk}{{\bf k}}
\newcommand{\bl}{{\bf l}}
% \newcommand{\bm}{{\bf m}}
\newcommand{\bn}{{\bf n}}
\newcommand{\bp}{{\bf p}}
\newcommand{\bq}{{\bf q}}
\newcommand{\br}{{\bf r}}
\newcommand{\bs}{{\bf s}}
\newcommand{\bt}{{\bf t}}
\newcommand{\bu}{{\bf u}}
\newcommand{\bv}{{\bf v}}
\newcommand{\bw}{{\bf w}}
\newcommand{\bx}{{\bf x}}
\newcommand{\by}{{\bf y}}
\newcommand{\bz}{{\bf z}}
\newcommand{\bzero}{{\bf0}}
\newcommand{\bone}{{\bf1}}
\newcommand{\btwo}{{\bf2}}
\newcommand{\bthree}{{\bf3}}
\newcommand{\bfour}{{\bf4}}
\newcommand{\bfive}{{\bf5}}
\newcommand{\bsix}{{\bf6}}
\newcommand{\bseven}{{\bf7}}
\newcommand{\beight}{{\bf8}}
\newcommand{\bnine}{{\bf9}}


% Other macros for regparam and iteration idx
\newcommand{\regparam}{\mu}
\newcommand{\itidx}{\ell}



\usepackage[round]{natbib}  % Use 'round' for (Author, Year) style, or 'numbers' if you want [1]
\usepackage{url}
\usepackage[utf8]{inputenc} % Input encoding
\usepackage[T1]{fontenc}    % Font encoding
\usepackage{amsmath}        % For math environments
\usepackage{amssymb} 
\usepackage{graphicx}
\usepackage[margin=1in]{geometry}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{amsmath}
\usepackage{enumitem}% For math symbols
\usepackage{amsfonts}       % For \mathbb
\usepackage{graphicx}       % To include graphics (optional for outline, but good for final)
\usepackage[margin=1in]{geometry} % Set margins
\usepackage[svgnames]{xcolor} % Use colors, svgnames provides more predefined names
\usepackage{titlesec}       % To customize section titles
\usepackage{hyperref} 
\usepackage{amsmath}
\usepackage{url}
\usepackage{bm}
\usepackage{algorithm}
\usepackage{algpseudocode}
\usepackage{cite}
\usepackage{graphicx}  % Required for \includegraphics
\usepackage{subcaption} % Required for the subfigure environment
\usepackage{float}     % For [H] placement (optional, if you need precise placement)
% \newcommand{\vx}{\mathbf{x}}
% \newcommand{\vy}{\mathbf{y}}
% \newcommand{\vH}{\mathbf{H}}
% \newcommand{\vR}{\mathbf{R}}
% \newcommand{\vQ}{\mathbf{Q}}
% \newcommand{\vM}{\mathbf{M}}
% \newcommand{\vC}{\mathbf{C}}
% \newcommand{\vP}{\mathbf{P}}
% \newcommand{\vS}{\mathbf{S}}
% \newcommand{\vU}{\mathbf{U}}
% \newcommand{\vI}{\mathbf{I}}
% \newcommand{\vB}{\mathbf{B}}
% \newcommand{\vA}{\mathbf{A}}
% \newcommand{\vD}{\mathbf{D}}
% \newcommand{\vK}{\mathbf{K}}
% \newcommand{\vL}{\mathbf{L}}
% \newcommand{\vG}{\mathbf{G}}
% \newcommand{\vT}{\mathbf{T}}
% \newcommand{\vN}{\mathbf{N}}
% \newcommand{\vE}{\mathbf{E}}
% \newcommand{\vZ}{\mathbf{Z}}
% \newcommand{\vW}{\mathbf{W}}
% \newcommand{\vxi}{\boldsymbol{\xi}} % Use boldsymbol for Greek letters
% \newcommand{\vepsilon}{\boldsymbol{\epsilon}} % Use boldsymbol for Greek letters
% \newcommand{\vmu}{\boldsymbol{\mu}} % Use boldsymbol for Greek letters
% \newcommand{\valpha}{\boldsymbol{\alpha}} % Use boldsymbol for Greek letters
% \newcommand{\vGamma}{\boldsymbol{\Gamma}} % Use boldsymbol for Greek letters

% Include other packages and settings from your preamble if necessary
% \usepackage[utf8]{inputenc}
% \usepackage{epsfig}
\usepackage{amssymb}
\usepackage{enumitem} % For condensed lists
\usepackage[margin=1in]{geometry} % Optional: Adjust margins
% \usepackage{amsthm} % For theorem and definition environments
\usepackage{mathrsfs} % For mathscr% For clickable links (TOC, citations - optional)
\hypersetup{
    colorlinks=true,
    linkcolor=black,
    citecolor=black,
    filecolor=magenta,      
    urlcolor=black,
    pdftitle={Kalman Filter with EM and OF},
    pdfpagemode=FullScreen
    }

%%%% HELPER CODE FOR DEALING WITH EXTERNAL REFERENCES ON OVERLEAF
% (from an answer by cyberSingularity at http://tex.stackexchange.com/a/69832/226)
%%%
\makeatletter
\newcommand*{\addFileDependency}[1]{% argument=file name and extension
  \typeout{(#1)}% latexmk will find this if $recorder=0 (however, in that case, it will ignore #1 if it is a .aux or .pdf file etc and it exists! if it doesn't exist, it will appear in the list of dependents regardless)
  \@addtofilelist{#1}% if you want it to appear in \listfiles, not really necessary and latexmk doesn't use this
  \IfFileExists{#1}{}{\typeout{No file #1.}}% latexmk will find this message if #1 doesn't exist (yet)
}
\makeatother

\newcommand*{\myexternaldocument}[1]{%
    \externaldocument{#1}%
    \addFileDependency{#1.tex}%
    \addFileDependency{#1.aux}%
}
%%% END HELPER CODE

%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 
